SwiFT: Swin 4D fMRI Transformer

Modeling spatiotemporal brain dynamics from high-dimensional data, such as functional Magnetic Resonance Imaging (fMRI), is a formidable task in neuroscience. Existing approaches for fMRI analysis utilize hand-crafted features, but the process of feature extraction risks losing essential information in fMRI scans. To address this challenge, we present SwiFT (Swin 4D fMRI Transformer), a Swin Transformer architecture that can learn brain dynamics directly from fMRI volumes in a memory and computation-efficient manner. SwiFT achieves this by implementing a 4D window multi-head self-attention mechanism and absolute positional embeddings. We evaluate SwiFT using multiple large-scale resting-state fMRI datasets, including the Human Connectome Project (HCP), Adolescent Brain Cognitive Development (ABCD), and UK Biobank (UKB) datasets, to predict sex, age, and cognitive intelligence. Our experimental outcomes reveal that SwiFT consistently outperforms recent state-of-the-art models. Furthermore, by leveraging its end-to-end learning capability, we show that contrastive loss-based self-supervised pre-training of SwiFT can enhance performance on downstream tasks. Additionally, we employ an explainable AI method to identify the brain regions associated with sex classification. To our knowledge, SwiFT is the first Swin Transformer architecture to process dimensional spatiotemporal brain functional data in an end-to-end fashion. Our work holds substantial potential in facilitating scalable learning of functional brain imaging in neuroscience research by reducing the hurdles associated with applying Transformer models to high-dimensional fMRI.

==> supple_tab_fig/table1.tex <==

\begin{table}
\caption{
% 
Efficiency comparison of different position embedding methods
% \textbf{.}
% 
} % \caption
\centering

\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lllllll}

\toprule
\multicolumn{1}{c}{\multirow{1}{*}{Method}} &
  \multicolumn{1}{c}{\# param.} &
  \multicolumn{1}{c}{FLOPs} &
  \multicolumn{1}{c}{throughput} \\
  \midrule
% SwiFT-rel (HCP)   & 2.059M & 1.73G  &  103.84  \\ 
% SwiFT-abs (HCP)   & 1.971M & 1.73G  &   117.61 \\
% SwiFT-rel (ABCD)   & 4.668M & 2.62G  &   94.17  \\ 
% SwiFT-abs (ABCD)   & 4.649M & 2.62G  &   104.46  \\ 
SwiFT-rel (HCP)   & 2.05M & 1.73G  &  103.84  \\ 
SwiFT-abs (HCP)   & 1.97M & 1.73G  &   117.61 \\
SwiFT-rel (ABCD)   & 4.66M & 2.62G  &   94.17  \\ 
SwiFT-abs (ABCD)   & 4.64M & 2.62G  &   104.46  \\
\bottomrule
\end{tabular}} %\resizebox
\label{tab:result3}
\end{table}

==> tab/table1.tex <==
\begin{table}
\caption{
% 
\textbf{Classification (sex) and Regression (age, intelligence) results of ABCD}
% 
} % \caption
\centering

\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lcccccc}

\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Method}} &
  \multicolumn{2}{c}{sex} &
  \multicolumn{2}{c}{age} &
  \multicolumn{2}{c}{intelligence} \\
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{Acc.} &
  \multicolumn{1}{c}{AUC} &
  \multicolumn{1}{c}{MSE} &
  \multicolumn{1}{c}{MAE} &
  \multicolumn{1}{c}{MSE} &
  \multicolumn{1}{c}{MAE} \\ 
  \midrule
  
XGBoost & 0.695 & 0.767 & 61.65 & 6.72 & 0.977 & 0.770  \\
BNT & \textbf{0.791}	& \textbf{0.889} & 52.53 & 6.15 & 0.955 & 0.767 \\
TFF & 0.738 & 0.802 & 54.92 & 6.42 & 0.968 & 0.768  \\
SwiFT (Ours)   & 75.9\tiny$\pm$1.6 & 84.7{\tiny$\pm$0.9}  &  \textbf{24.09{\tiny$\pm$0.50}}  & \textbf{3.83{\tiny$\pm$0.06}}  &    \textbf{0.446{\tiny$\pm$0.02}} & \textbf{0.407{\tiny$\pm$0.02}} \\ 
\bottomrule
\end{tabular}} % \resizebox
\label{tab:result1}
\end{table}


==> tab/table2.tex <==
\begin{table}
\caption{
% 
\textbf{Classification (sex) and Regression (age, intelligence) results of HCP}
% 
} % \caption
\centering
% \begin{tabular}{@{}lcccc@{}}
% \toprule
% Method & Accuracy & AUC \\
% \midrule
% baseline(ML) & 00.5\% & 00.3\% \\
% baseline(simpleCNN) & 57.2\% & 00.3\%   \\
% baseline(VGGnet11) & 57.2\% & 00.3\%   \\
% Ours(alpha+f) & 57.2\% & 00.3\% \\
% Ours(CCE+f) & 57.2\% & 00.3\% \\

% \bottomrule
% Please add the following required packages to your document preamble:

\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lllllll}

\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Method}} &
  \multicolumn{2}{c}{sex} &
  \multicolumn{2}{c}{age} &
  \multicolumn{2}{c}{intelligence} \\
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{Acc.} &
  \multicolumn{1}{c}{AUC} &
  \multicolumn{1}{c}{MSE} &
  \multicolumn{1}{c}{MAE} &
  \multicolumn{1}{c}{MSE} &
  \multicolumn{1}{c}{MAE} \\ 
  \midrule
  
XGBoost & 0.685 & 0.755 & 14.31 & 3.12 & 0.991 & 0.813  \\
BNT & 0.810	& 0.880 & 12.77 & 2.98 & 1.001 & 0.830 \\
TFF & 0.925 & 0.975 & 13.77 & 3.11 & 0.953 & 0.795  \\
SwiFT (Ours)   & 0.923 & \textbf{0.981}  &  4.90  & \textbf{1.62}  &    0.361 & \textbf{0.368} \\ 
\bottomrule
\end{tabular}} % \resizebox
\label{tab:result2}
\end{table}


==> tab/table4.tex <==
\begin{tabular}{lcccccc}

\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Loss Function}} &
  \multicolumn{2}{c}{Sex} &
  \multicolumn{2}{c}{Age (Month)} &
  \multicolumn{2}{c}{Intelligence} \\
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{Acc.(\%)} &
  \multicolumn{1}{c}{AUC(\%)} &
  \multicolumn{1}{c}{MSE} &
  \multicolumn{1}{c}{MAE} &
  \multicolumn{1}{c}{MSE} &
  \multicolumn{1}{c}{MAE} \\ 
  \midrule
  
No pre-training & 74.1 & 83.5 & \textbf{23.81} & 3.827 & \textbf{0.457} & 0.425  \\
IC & 77.3	& 85.6 & 25.01 & 3.697 & 0.472 & 0.401 \\
LL & 78.4 & 86.7 & 24.87 & \textbf{3.413} & 0.473 & 0.352  \\
IC + LL & \textbf{79.8} & \textbf{87.6}  &  24.95  & 3.414  &    0.474 & \textbf{0.351} \\ 
\bottomrule
\end{tabular}

==> tab/table_combined_backup.tex <==


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[t]
% \caption{Performance comparison between baselines}
% \centering
% \begin{tabular}{c|cccccc|cccccc}
% \hline
% \multirow{3}{*}{Method} & \multicolumn{6}{c|}{ABCD} & \multicolumn{6}{c}{HCP} \\ \cline{2-13} 
%  & \multicolumn{2}{c}{Sex} & \multicolumn{2}{c}{Age} & \multicolumn{2}{c|}{Intelligence} & \multicolumn{2}{c}{Sex} & \multicolumn{2}{c}{Age} & \multicolumn{2}{c}{Intelligence} \\
%                         & ACC        & AUROC      & MSE             & MAE           & MSE                & MAE               & ACC        & AUROC      & MSE             & MAE           & MSE                & MAE               \\ \hline
% XGBoost                 & 69.5       & 76.7       & 61.65           & 6.72          & 0.977              & 0.770             & 68.5       & 75.5       & 14.31           & 3.12          & 0.991              & 0.813             \\
% Brain CNN               & 80.1       & 87.9       & 53.19           & 6.04          & 0.969              & 0.767             & 77.1       & 84.9       & 12.63           & 2.97          & 0.984              & 0.805             \\
% Graphormer              & 77.4       & 85.1       & 52.45           & 6.05          & 0.961              & 0.764             & 77.9       & 85.2       & 12.53           & 2.95          & 0.987              & 0.812             \\
% BNT                     & 79.1       & 88.9       & 52.53           & 6.15          & 0.955              & 0.767             & 81.0       & 88.0       & 12.77           & 2.98          & 1.001              & 0.830             \\
% TFF                     & 73.8       & 80.2       & 54.92           & 6.42          & 0.968              & 0.768             & 92.5       & 97.5       & 13.77           & 3.11          & 0.953              & 0.795             \\
% Swin                    & 75.9       & 84.7       & 24.09           & 3.83          & 0.446              & 0.407             & 92.3       & 98.1       & 4.90            & 1.62          & 0.361              & 0.368            \\ \hline
% \end{tabular}
% \end{table*}










% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\caption{Performance comparison to baselines on classification and regression tasks}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccccc|cccccc}
\hline
\multicolumn{1}{c|} {\multirow{3}{*}{Method}} & \multicolumn{6}{c|}{ABCD} & \multicolumn{6}{c}{HCP} \\ \cline{2-13} 
\multicolumn{1}{c|}{} & \multicolumn{2}{c}{Sex} & \multicolumn{2}{c}{Age (Month)} & \multicolumn{2}{c|}{Intelligence} & \multicolumn{2}{c}{Sex} & \multicolumn{2}{c}{Age (Year)} & \multicolumn{2}{c}{Intelligence} \\
\multicolumn{1}{c|}{}                        & ACC (\%)        & AUC (\%)      & MSE             & MAE           & MSE                & MAE               & ACC (\%)        & AUC (\%)      & MSE             & MAE           & MSE                & MAE               \\ \hline
XGBoost \cite{chen2016xgboost}   & 69.5$_{\pm0.6}$ & 76.7$_{\pm0.9}$ & 61.65$_{\pm0.45}$ & 6.72$_{\pm0.05}$ & 0.977$_{\pm0.037}$ & 0.770$_{\pm0.016}$  & 68.5$_{\pm3.0}$ & 75.5$_{\pm3.1}$ & 14.31$_{\pm1.61}$ & 3.12$_{\pm0.20}$ & 0.991$_{\pm0.084}$ & 0.813$_{\pm0.032}$ \\
BrainNetCNN \cite{kawahara2017brainnetcnn}  & \textbf{80.1}$_{\pm0.7}$ & 87.9$_{\pm0.4}$ & 53.19$_{\pm1.26}$ & 6.04$_{\pm0.19}$ & 0.969$_{\pm0.042}$ & 0.767$_{\pm0.016}$ & 77.1$_{\pm0.2}$ & 84.9$_{\pm0.0}$ & 12.63$_{\pm0.74}$ & 2.97$_{\pm0.15}$ & 0.984$_{\pm0.034}$ & 0.805$_{\pm0.016}$ \\
Graphormer \cite{ying2021transformers} & 77.4$_{\pm2.5}$ & 85.1$_{\pm3.2}$ & 52.45$_{\pm0.86}$ & 6.05$_{\pm0.18}$ & 0.961$_{\pm0.050}$ & 0.764$_{\pm0.025}$ & 77.9$_{\pm2.1}$ & 85.2$_{\pm0.9}$ & 12.53$_{\pm1.15}$ & 2.95$_{\pm0.18}$ & 0.987$_{\pm0.039}$ & 0.812$_{\pm0.014}$ \\
BNT \cite{kan2022bnt}        & 79.1$_{\pm2.5}$ & \textbf{88.9}$_{\pm0.6}$ & 52.53$_{\pm2.08}$ & 6.15$_{\pm0.12}$ & 0.955$_{\pm0.043}$ & 0.767$_{\pm0.018}$ & 81.0$_{\pm4.2}$   & 88$_{\pm3.1}$   & 12.77$_{\pm0.89}$ & 2.98$_{\pm0.15}$ & 1.001$_{\pm0.009}$ & 0.83$_{\pm0.014}$  \\
TFF \cite{malkiel2022self}        & 73.8$_{\pm1.1}$ & 80.2$_{\pm1.1}$ & 54.92$_{\pm1.67}$ & 6.42$_{\pm0.15}$ & 0.968$_{\pm0.024}$ & 0.768$_{\pm0.009}$ & \textbf{92.5}$_{\pm1.1}$ & 97.5$_{\pm1.4}$   & 13.77$_{\pm1.12}$ & 3.11$_{\pm0.20}$ & 0.953$_{\pm0.074}$ & 0.795$_{\pm0.028}$ \\ \hline
SwiFT (Ours)       & 75.9$_{\pm1.6}$ & 84.7$_{\pm0.9}$ & \textbf{24.09}$_{\pm0.50}$ & \textbf{3.83}$_{\pm0.06}$ & \textbf{0.446}$_{\pm0.019}$ & \textbf{0.407}$_{\pm0.021}$ & 92.3$_{\pm2.4}$ & \textbf{98.1}$_{\pm0.6}$   & \textbf{4.90}$_{\pm0.65}$   & \textbf{1.62}$_{\pm0.14}$ & \textbf{0.361}$_{\pm0.033}$ & \textbf{0.368}$_{\pm0.029}$ \\ \hline
% \multicolumn{13}{c}{Only split 1} \\\hline
% SwiFT (Pre-trained)* & 79.8  & 87.6  & 24.95 & 3.414 & 0.474 & 0.351 & -   & -   & - & -  & -  & -  \\\hline
\end{tabular}
}
% \captionsetup{singlelinecheck = false, format= hang, justification=raggedright, font=footnotesize, labelsep=space}
% \caption*{\scriptsize *Trained and evaluated only on one of the three data splits due to time constraints.}
\label{tab:result_combined}
\end{table*}



==> tab/table_combined_backup_new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\caption{Performance comparison to baselines on classification and regression tasks}
\centering
\resizebox{1.1\linewidth}{!}{
\begin{tabular}{l|cccc|cccccc|cccccc}
\hline
\multirow{3}{*}{Method} & \multicolumn{4}{c|}{ABCD}                                         & \multicolumn{6}{c|}{HCP}                                                                           & \multicolumn{6}{c}{UKB}                       \\ \cline{2-17} 
                        & \multicolumn{2}{c}{Sex} & \multicolumn{2}{c|}{Total intelligence} & \multicolumn{2}{c}{Sex} & \multicolumn{2}{c}{Age (year)} & \multicolumn{2}{c|}{Total intelligence} & \multicolumn{2}{c}{Sex} & \multicolumn{2}{c}{Age (year)} & \multicolumn{2}{c}{Fluid intelligence} \\
                        & ACC        & AUROC      & MSE                & MAE               & ACC        & AUROC      & MSE            & MAE           & MSE                & MAE               & ACC        & AUROC      & MSE            & MAE           & MSE                & MAE               \\ \hline
XGBoost                 & 69.5       & 76.7       & 0.977              & 0.770             & 68.5       & 75.5       & 14.3           & 3.12          & 0.991              & 0.813             & 79.5       & 87.6       & 48.8           & 5.85          & 1.055              & 0.816             \\ 
BrainNetCNN\cite{kawahara2017brainnetcnn}               & \textbf{80.1}       & 87.9       & 0.969              & 0.767             & 77.1       & 84.9       & 12.6           & 2.97          & 0.984              & 0.805             & 86.8       & 93.8       & 42.7           & 5.36          & 1.001              & 0.800             \\ 
VanillaTF\cite{kan2022bnt}              & 77.4       & 85.1       & 0.961              & 0.764             & 77.9       & 85.2       & 12.5           & 2.95          & 0.987              & 0.812             & 87.0       & 95.1       & 41.4           & 5.26          & 0.999              & 0.799             \\ 
BNT\cite{kan2022bnt}                     & 79.1       & \textbf{88.9}       & 0.955              & 0.767             & 81.0       & 88.0       & 12.8           & 2.98          & 1.001              & 0.830             & 87.0       & 94.8       & 39.6           & 5.17          & 0.998              & 0.798             \\ 
TFF\cite{malkiel2022self}                     & 73.8       & 80.2       & 0.968              & 0.768             & \textbf{92.5}       & 97.5       & 13.8           & 3.11          & 0.953              & 0.795             & 96.8       & 99.5       & 42.1           & 5.10          & 0.997              & \textbf{0.783}             \\ \hline
SwiFT (ours)                    & 79.3       & 87.8       &\textbf{ 0.932}              & \textbf{0.756}             & 92.3       & \textbf{98.1}       & \textbf{8.6}            & \textbf{2.36 }         & \textbf{0.871}              & \textbf{0.776}             & \textbf{97.7 }      & \textbf{99.8}       & \textbf{18.2 }          & \textbf{3.40}          & \textbf{0.992}              & 0.796            \\
\hline
\end{tabular}
}
% \captionsetup{singlelinecheck = false, format= hang, justification=raggedright, font=footnotesize, labelsep=space}
% \caption*{\scriptsize *Trained and evaluated only on one of the three data splits due to time constraints.}
\label{tab:result_combined}
\end{table*}





==> tab/table_combined_previous_main_results.tex <==


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[t]
% \caption{Performance comparison between baselines}
% \centering
% \begin{tabular}{c|cccccc|cccccc}
% \hline
% \multirow{3}{*}{Method} & \multicolumn{6}{c|}{ABCD} & \multicolumn{6}{c}{HCP} \\ \cline{2-13} 
%  & \multicolumn{2}{c}{Sex} & \multicolumn{2}{c}{Age} & \multicolumn{2}{c|}{Intelligence} & \multicolumn{2}{c}{Sex} & \multicolumn{2}{c}{Age} & \multicolumn{2}{c}{Intelligence} \\
%                         & ACC        & AUROC      & MSE             & MAE           & MSE                & MAE               & ACC        & AUROC      & MSE             & MAE           & MSE                & MAE               \\ \hline
% XGBoost                 & 69.5       & 76.7       & 61.65           & 6.72          & 0.977              & 0.770             & 68.5       & 75.5       & 14.31           & 3.12          & 0.991              & 0.813             \\
% Brain CNN               & 80.1       & 87.9       & 53.19           & 6.04          & 0.969              & 0.767             & 77.1       & 84.9       & 12.63           & 2.97          & 0.984              & 0.805             \\
% Graphormer              & 77.4       & 85.1       & 52.45           & 6.05          & 0.961              & 0.764             & 77.9       & 85.2       & 12.53           & 2.95          & 0.987              & 0.812             \\
% BNT                     & 79.1       & 88.9       & 52.53           & 6.15          & 0.955              & 0.767             & 81.0       & 88.0       & 12.77           & 2.98          & 1.001              & 0.830             \\
% TFF                     & 73.8       & 80.2       & 54.92           & 6.42          & 0.968              & 0.768             & 92.5       & 97.5       & 13.77           & 3.11          & 0.953              & 0.795             \\
% Swin                    & 75.9       & 84.7       & 24.09           & 3.83          & 0.446              & 0.407             & 92.3       & 98.1       & 4.90            & 1.62          & 0.361              & 0.368            \\ \hline
% \end{tabular}
% \end{table*}










% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\caption{Performance comparison to baselines on classification and regression tasks}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccccc|cccccc}
\hline
\multicolumn{1}{c|} {\multirow{3}{*}{Method}} & \multicolumn{6}{c|}{HCP} & \multicolumn{6}{c}{ABCD} \\ \cline{2-13} 
\multicolumn{1}{c|}{} & \multicolumn{2}{c}{Sex} & \multicolumn{2}{c}{Age (Year)} & \multicolumn{2}{c|}{Intelligence} & \multicolumn{2}{c}{Sex} & \multicolumn{2}{c}{Age (Month)} & \multicolumn{2}{c}{Intelligence} \\
\multicolumn{1}{c|}{}                        & ACC (\%)        & AUC (\%)      & MSE             & MAE           & MSE                & MAE               & ACC (\%)        & AUC (\%)      & MSE             & MAE           & MSE                & MAE               \\ \hline
XGBoost \cite{chen2016xgboost}   & 68.5$_{\pm3.0}$ & 75.5$_{\pm3.1}$ & 14.31$_{\pm1.61}$ & 3.12$_{\pm0.20}$ & 0.991$_{\pm0.084}$ & 0.813$_{\pm0.032}$ & 69.5$_{\pm0.6}$ & 76.7$_{\pm0.9}$ & 61.65$_{\pm0.45}$ & 6.72$_{\pm0.05}$ & 0.977$_{\pm0.037}$ & 0.770$_{\pm0.016}$  \\
BrainNetCNN \cite{kawahara2017brainnetcnn}  & 77.1$_{\pm0.2}$ & 84.9$_{\pm0.0}$ & 12.63$_{\pm0.74}$ & 2.97$_{\pm0.15}$ & 0.984$_{\pm0.034}$ & 0.805$_{\pm0.016}$ & \textbf{80.1}$_{\pm0.7}$ & 87.9$_{\pm0.4}$ & 53.19$_{\pm1.26}$ & 6.04$_{\pm0.19}$ & 0.969$_{\pm0.042}$ & 0.767$_{\pm0.016}$ \\
Graphormer \cite{ying2021transformers}  & 77.9$_{\pm2.1}$ & 85.2$_{\pm0.9}$ & 12.53$_{\pm1.15}$ & 2.95$_{\pm0.18}$ & 0.987$_{\pm0.039}$ & 0.812$_{\pm0.014}$ & 77.4$_{\pm2.5}$ & 85.1$_{\pm3.2}$ & 52.45$_{\pm0.86}$ & 6.05$_{\pm0.18}$ & 0.961$_{\pm0.050}$ & 0.764$_{\pm0.025}$\\
BNT \cite{kan2022bnt}        & 81.0$_{\pm4.2}$   & 88.0$_{\pm3.1}$   & 12.77$_{\pm0.89}$ & 2.98$_{\pm0.15}$ & 1.001$_{\pm0.009}$ & 0.830$_{\pm0.014}$ & 79.1$_{\pm2.5}$ & \textbf{88.9}$_{\pm0.6}$ & 52.53$_{\pm2.08}$ & 6.15$_{\pm0.12}$ & 0.955$_{\pm0.043}$ & 0.767$_{\pm0.018}$  \\
TFF \cite{malkiel2022self}        & \textbf{92.5}$_{\pm1.1}$ & 97.5$_{\pm1.4}$   & 13.77$_{\pm1.12}$ & 3.11$_{\pm0.20}$ & 0.953$_{\pm0.074}$ & 0.795$_{\pm0.028}$ & 73.8$_{\pm1.1}$ & 80.2$_{\pm1.1}$ & 54.92$_{\pm1.67}$ & 6.42$_{\pm0.15}$ & 0.968$_{\pm0.024}$ & 0.768$_{\pm0.009}$ \\ \hline
SwiFT (Ours)       & 92.3$_{\pm2.4}$ & \textbf{98.1}$_{\pm0.6}$   & \textbf{4.90}$_{\pm0.65}$   & \textbf{1.62}$_{\pm0.14}$ & \textbf{0.361}$_{\pm0.033}$ & \textbf{0.368}$_{\pm0.029}$ & 75.9$_{\pm1.6}$ & 84.7$_{\pm0.9}$ & \textbf{24.09}$_{\pm0.50}$ & \textbf{3.83}$_{\pm0.06}$ & \textbf{0.446}$_{\pm0.019}$ & \textbf{0.407}$_{\pm0.021}$  \\ \hline
% \multicolumn{13}{c}{Only split 1} \\\hline
% SwiFT (Pre-trained)* & 79.8  & 87.6  & 24.95 & 3.414 & 0.474 & 0.351 & -   & -   & - & -  & -  & -  \\\hline
\end{tabular}
}
% \captionsetup{singlelinecheck = false, format= hang, justification=raggedright, font=footnotesize, labelsep=space}
% \caption*{\scriptsize *Trained and evaluated only on one of the three data splits due to time constraints.}
\label{tab:result_combined}
\end{table*}


